A congruence modulo four in real Schubert calculus

We establish a congruence modulo four in the real Schubert calculus on the Grassmannian of m-planes in 2m-space. This congruence holds for fibers of the Wronski map and a generalization to what we call symmetric Schubert problems. This strengthens the usual congruence modulo two for numbers of real solutions to geometric problems. It also gives examples of geometric problems given by fibers of a map whose topological degree is zero but where each fiber contains real points.

==> pictures/files <==
1.eps    \I   A workhorse
1s.eps   \Is  Just for subscripts
21s.eps    \TI
22s.eps    \TT
311s.eps   \ThII
321.eps   \ThTI
332s.eps  \ThThT
333s.eps  \ThThTh

 322.eps     \ThTT  Used in displayed formulas
 331.eps     Used in displayed formulas

These are each used once in a displayed formula
 21.eps      
 4211.eps    
 52s.eps     
 53211.eps
 53211D.eps
 3211.eps
 421.eps
 311_21.4.eps
 332_321.5.eps


